GigaWorld-Policy: An Efficient Action-Centered World--Action Model

World-Action Models (WAM) initialized from pre-trained video generation backbones have demonstrated remarkable potential for robot policy learning. However, existing approaches face two critical bottlenecks that hinder performance and deployment. First, jointly reasoning over future visual dynamics and corresponding actions incurs substantial inference overhead. Second, joint modeling often entangles visual and motion representations, making motion prediction accuracy heavily dependent on the quality of future video forecasts. To address these issues, we introduce GigaWorld-Policy, an action-centered WAM that learns 2D pixel-action dynamics while enabling efficient action decoding, with optional video generation. Specifically, we formulate policy training into two coupled components: the model predicts future action sequences conditioned on the current observation, and simultaneously generates future videos conditioned on the predicted actions and the same observation. The policy is supervised by both action prediction and video generation, providing richer learning signals and encouraging physically plausible actions through visual-dynamics constraints. With a causal design that prevents future-video tokens from influencing action tokens, explicit future-video generation is optional at inference time, allowing faster action prediction during deployment. To support this paradigm, we curate a diverse, large-scale robot dataset to pre-train an action-centered video generation model, which is then adapted as the backbone for robot policy learning. Experimental results on real-world robotic platforms show that GigaWorld-Policy runs 9x faster than the leading WAM baseline, Motus, while improving task success rates by 7%. Moreover, compared with pi-0.5, GigaWorld-Policy improves performance by 95% on RoboTwin 2.0.

==> sections/GigaBrain_Data.tex <==

% % \begin{table}[t]
% % \centering
% % \captionsetup{type=table, justification=justified, singlelinecheck=false}
% % \caption{Comparison of training data usage across VLA models. \textit{GigaBrain-0} leverages a diverse set of data sources to enhance generalization and reduce dependency on real-world robot data.}
% % \label{tab:data_support}
% % \begin{tabular}{l *{7}{>{\centering\arraybackslash}m{1.55cm}}}
% % \toprule
% % {Method} & 
% % \rot{Public Data} &
% % \rot{Self-Collected Data} &
% % \rot{Egocentric Human Data} &
% % \rot{Video-Gen Data} &
% % \rot{Sim2Real Transfer Data} &
% % \rot{Real2Real Transfer Data} &
% % \rot{View Transfer Data} \\
% % \midrule
% % $\pi_0$            & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
% % $\pi_{0.5}$          & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
% % G0       & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
% % WALL-OSS       & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
% % GR-3           & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark \\
% % GR00T N1.5    & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark \\
% % \midrule
% % \textbf{\textit{GigaBrain-0}}    & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
% % \bottomrule
% % \end{tabular}
% % \end{table}

% \section{GigaBrain-0 Data}
% \label{sec:data}
% For Vision-Language-Action (VLA) models, training data diversity is paramount~\citep{shi2025diversity}. While numerous public datasets~\citep{oxe,robomind,agibot} exist, they are often insufficient in scene variation, or task complexity to enable robust generalization. Real-world robot data collection suffers from high operational costs, low scaling efficiency, and limited environmental diversity, as most deployments repeatedly sample from the same narrow set of scenes.


% Recent advances~\citep{gr00t,dreamgen} have demonstrated that world models can effectively generate diverse and photorealistic training data to augment vision-language-action (VLA) capabilities. In \textit{GigaBrain-0}, we further extend this paradigm by integrating a broad spectrum of world-model-generated data sources. As shown in Tab.~\ref{tab:data_support}, \textit{GigaBrain-0} leverages a more diverse set of data sources compared to existing VLA counterparts~\citep{pi0,pi05,walloss,galaxea,gr3,gr00t}. This expanded data diversity significantly reduces reliance on real-world robot-collected data while enhancing model generalization. We detail each data source in the following.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1\linewidth]{images/realdata.pdf}
%     \captionsetup{type=figure, justification=justified, singlelinecheck=false}
%     \caption{\textit{GigaBrain-0}'s self-collected real-world robot data is gathered from PiPER arms and the AgiBot G1 platform, spanning diverse environments including homes, supermarkets, factories, and office settings.}
%     \label{fig:real_data}
% \end{figure}

% \subsection{Real-World Data}
% \label{subsec:real_data}

% \textbf{Data Source}. Our real-world data corpus integrates both publicly available datasets and proprietary data collected from our in-house robotic platforms. Publicly sourced datasets include AgiBotWorld~\citep{agibot}, RoboMind~\citep{robomind}, and Open X-Embodiment~\citep{oxe}, which collectively provide foundational coverage of manipulation and locomotion tasks. 
% In addition, we collect 1182 hours proprietary data using Agilex Cobot Magic platform (199 hours) and the AgiBot G1 platform (983 hours) across a total area of 3100$\text{m}^2$, spanning five broad environment categories: industrial, commercial, office, residential, and laboratory settings. These are further subdivided into 14 distinct real-world scenarios, including supermarkets, hotel lobbies, coffee shops, bubble tea stores, convenience stores, restaurants, warehouse material handling, industrial assembly lines, pantries, private residences, apartment interiors, meeting rooms, office workstations, and laboratories.
% The collected tasks range from basic pick-and-place operations to long-horizon sequential activities, mobile manipulation in dynamically changing layouts, and interactions with deformable objects, as illustrated in Fig.~\ref{fig:real_data}.


% \textbf{Data Annotation \& Processing}. 
% For data annotation, if the captured RGB frames lack depth information, we employ MoGe~\citep{moge} to generate metrically scaled depth maps. Regarding subgoal language annotation, we observe that VLMs struggle to accurately segment long-horizon tasks into meaningful subgoals, while manual segmentation proves prohibitively time-consuming. To address this, we adopt an approach inspired by~\citep{rlbench}, leveraging gripper state transitions (e.g., open/close, grasp/release) to automatically segment trajectories into atomic subtasks.
% For each segmented subtask, we utilize Qwen-VL-2.5~\citep{qwen25vl} to generate subgoal language annotations. To mitigate hallucination and ensure consistency, we constrain the annotation process using a structured template and a predefined vocabulary of standardized action phrases (e.g., \texttt{pick [object]}, \texttt{place [object] into [container]}, \texttt{open [device]}), selected from a curated description library.
% For 2D manipulation trajectory annotation, we project the 3D end-effector coordinates into the head-mounted camera’s image plane, yielding pixel-space motion traces aligned with visual observations.
% Notably, we annotate only a subset of the collected data and train our models using a mixture of fully annotated, partially annotated, and raw unannotated trajectories to maximize data utility while managing annotation costs.
% To further improve pretraining efficiency and reduce redundancy, we perform deduplication across the entire corpus. For each unique task, we retain at most 50 diverse demonstration trajectories, preserving behavioral variety while eliminating near-identical repetitions. This strategy enhances sample efficiency and promotes more robust and generalizable model learning.




% \subsection{World-Model-Generated Data}
% \label{subsec:synthetic_data}

% To overcome the limitations of physical data collection, we employ GigaWorld, our world-model framework, to generate diverse, physically plausible training sequences. GigaWorld synthesizes data through multiple complementary pipelines:

% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/real2real.pdf}
% \caption{GigaWorld enables Real2Real apperance transfer by taking real-world captured data and generating generalized variations in texture, color, lighting, and material properties.}
% \label{fig:real2real}
% \end{figure}

% \textbf{Real2Real Transfer}. Real-world robot-collected videos are inherently constrained by the physical environments in which they are captured, including static backgrounds, fixed lighting conditions, and limited variation in object materials, textures, and colors. To overcome these limitations and significantly enhance visual and contextual diversity, we leverage GigaWorld to perform Real2Real Transfer: re-rendering real trajectories in synthetically altered but physically plausible visual contexts. Specifically, we train diffusion-based video generation model~\citep{emma,robotransfer} conditioned on geometric and structural priors extracted from real footage. We employ VideoDepthAnything~\citep{videodepth} to estimate per-frame depth maps and extract Canny edge maps to preserve object boundaries and scene structure. These signals serve as spatial control conditions via a ControlNet~\citep{controlnet} branch, enabling precise manipulation of appearance while preserving motion and layout consistency. During inference, for each real-world video clip, we generate approximately 10 visually distinct variants by textually prompting changes to foreground/background materials, surface textures, illumination conditions, and color palettes, all while maintaining the original action semantics and spatial dynamics, as shown in Fig.~\ref{fig:real2real}. This approach efficiently multiplies the effective diversity of real data without requiring additional physical collection.

% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/viewtransfer.pdf}
% \caption{GigaWorld supports view transfer by re-rendering real-world captured data from diverse viewpoints, thereby enriching the dataset with varied perspective changes.}
% \label{fig:view_transfer}
% \end{figure}

% \textbf{View Transfer}.
% Beyond texture and illumination variation, generalization across observation viewpoints is equally critical for robust embodied perception~\citep{xing2025shortcut}. To this end, we exploit GigaWorld’s viewpoint generalization capability to augment real robot-collected data with novel camera perspectives while preserving 3D scene consistency.
% Specifically, to ensure geometric coherence under viewpoint changes, we project the original RGB frames into novel views using collected depth maps. If depth is unavailable in the source data, we annotate metric-scale depth using MoGe~\citep{moge}. The reprojected views inevitably contain occluded or incomplete regions, we inpaint these using a DiT-based video completion model~\citep{egodemogen} conditioned on the reprojected views.
% Notably, when the camera viewpoint shifts, the robot’s end-effector must remain functionally consistent with the task, even though its joint configuration changes. We compute the new joint angles via IK based on the updated ego-pose and end-effector pose. The resulting articulated robot geometry is then rendered using its URDF model in a physics-aware simulation engine, and provided as a structural condition~\citep{egodemogen} to the generative model.
% To mitigate potential discrepancies between simulated and real robot dynamics, we optionally employ a differentiable physics engine~\citep{embodiedreamer} to fine-tune motion plausibility and close the sim-to-real physics gap.
% As shown in Fig.~\ref{fig:view_transfer}, from a single real-world trajectory, our pipeline generates multiple viewpoint-consistent renderings of the scene, complete with dynamically adjusted robot poses that preserve task semantics and physical feasibility.


% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/sim2real.pdf}
% \caption{GigaWorld enables Sim2Real transfer by generalizing simulation-collected data in terms of texture, color, lighting, and material properties to better bridge the domain gap and enhance realism.}
% \label{fig:sim2real}
% \end{figure}

% \textbf{Sim2Real Transfer}.
% While the methods described above augment real-world data, we further scale our training corpus by leveraging simulation assets to synthesize diverse embodied interaction sequences. Specifically, we compose manipulation scenes in Isaac Sim~\citep{issacsim} using either procedurally generated assets from EmbodiedGen~\citep{embodiedgen} or curated objects from open-source repositories such as ArtVIP~\citep{artvip}. Robot morphology is defined via URDF files, and end-effector trajectories are computed using IK to ensure physically plausible motion.
% To bridge the sim-to-real domain gap, particularly in visual appearance, we apply GigaWorld’s Sim2Real Transfer pipeline. Similar in architecture to Real2Real Transfer, this method conditions a diffusion-based video generator~\citep{robotransfer,emma} on depth maps exported from the simulation environment. Using text prompts, we dynamically alter surface textures, material reflectance, lighting conditions, and environmental clutter to produce photorealistic renderings that retain the original scene geometry and action semantics, as illustrated in Fig.~\ref{fig:sim2real}.
% Crucially, unlike real-world data, simulation affords us full control over scene parameters: we can systematically vary object initial positions, camera viewpoints, background layouts, and even physics properties (e.g., friction, mass) to maximize combinatorial diversity.


% \begin{figure}[t]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/human_transfer.pdf}
% \caption{GigaWorld supports egocentric human video transfer by transforming first-person human hand actions into robotic manipulation scenarios, effectively mapping human demonstrations to robot-executable tasks.}
% \label{fig:human_transfer}
% \end{figure}


% \textbf{Human Video Transfer}. 
% Human demonstration videos have emerged as a promising source for training embodied agents~\citep{gr3,mimicplay,egovla,egomimic,bu2025univla}, offering diversity in tasks, environments, and interaction styles, far exceeding the scale and variety achievable through robotic data collection alone. However, raw human videos exhibit significant gaps when directly applied to robot learning, as egocentric footage often suffers from motion blur, unstable viewpoints, and a visual and kinematic mismatch between human hands and robotic end-effectors.
% To bridge this gap, we leverage GigaWorld’s video inpainting capabilities to transform large-scale first-person human videos into stable, robot-centric demonstrations. Specifically, we convert videos from the EgoDex dataset~\citep{egodex} into stabilized, robot-executable sequences with articulated mechanical arms replacing human hands. Specifically, we use SAM2~\citep{sam2} to segment and mask out human hands in each frame. The annotated 3D hand wrist positions (provided in EgoDex) are treated as target end-effector poses for a simulated robot arm. We solve for corresponding joint angles via IK, then render the robot’s URDF model using a physics-aware simulation engine. This rendered arm geometry serves as a structural condition for our diffusion-based generator~\citep{mimicdreamer}, ensuring kinematically plausible and visually consistent robot appearances.
% As shown in Fig.~\ref{fig:human_transfer}, the output is a stabilized, robot-embodied version of the original human demonstration, preserving task intent and spatial relationships while eliminating visual and kinematic domain gaps.


% \textbf{Video Generation with Inverse Dynamics Modeling}.
% Given a single input image, GigaWorld can generate diverse embodied robotic operation videos conditioned on different textual prompts, as illustrated in Fig.~\ref{fig:videogen}. Furthermore, we leverage Inverse Dynamics Models (IDM)~\citep{dreamgen} to infer corresponding robot action sequences from these generated videos, which are then used as synthetic training data for embodied manipulation tasks.

% \begin{figure}[t]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/videogen.pdf}
% \caption{GigaWorld can generate diverse future trajectories from the same initial frame under different text prompts, thereby augmenting the dataset with novel manipulation sequences.}
% \label{fig:videogen}
% \end{figure}


% \begin{figure}[t]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/mv.png}
% \caption{GigaWorld can generate multi-view consistent videos, thereby enabling 3D-aware training and improving spatial reasoning in downstream tasks.}
% \label{fig:mv}
% \end{figure}


% \textbf{Multiview Video Generation}.
% In embodied manipulation scenarios, multiple cameras (e.g., head-mounted and wrist-mounted cameras) are often deployed to capture the operating environment from different viewpoints, creating a demand for generating temporally and spatially consistent multiview videos. To address this, GigaWorld adopts the multiview modeling approach from~\citep{drivedreamer2,robotransfer,emma}, which concatenates noise maps from multiple views as input to the diffusion model. This design preserves the original diffusion architecture without modification and enables consistent multiview video generation with only minimal fine-tuning data. As shown in Fig.~\ref{fig:mv}, GigaWorld is capable of generating diverse yet geometrically consistent multiview videos, demonstrating strong cross-view coherence and scene fidelity.




% \textbf{Generation Efficiency}.
% Video diffusion models~\citep{cosmos,hunyuanvideo,wan} suffer from low generation efficiency, often requiring tens of minutes to synthesize hundreds of frames resolution. To accelerate inference, GigaWorld employs NATTEN~\citep{natten} as a computationally efficient alternative to standard self-attention. Furthermore, GigaWorld leverages step distillation~\citep{dmd2} to reduce the denoising process from dozens of steps to a single-step generation. Combined with FP8-precision inference, these optimizations collectively yield over a 50$\times$ speedup in video generation compared to baseline diffusion models.

% \textbf{Generated Data Quality Inspection}.
% Generated videos inevitably contain hallucinations or artifacts that may degrade downstream training performance. To mitigate this, GigaWorld introduces a comprehensive quality assessment pipeline that evaluates generated videos across multiple dimensions: geometric consistency~\citep{robotransfer}, multiview consistency~\citep{robotransfer}, text-description alignment~\citep{cosmosreason}, and physical plausibility~\citep{cosmosreason}. Each video is assigned a composite quality score, which determines whether it is suitable for pre-training, fine-tuning, or should be discarded. All model and training details mentioned above will be fully elaborated in the upcoming GigaWorld technical report.



==> sections/GigaBrain_Evaluation.tex <==
\section{Experiment}

To evaluate manipulation performance in real-world settings, we conduct experiments on a bimanual PiPER robot platform. Our evaluation spans a diverse set of task categories. In addition to task success, we benchmark the end-to-end policy inference latency and compare against representative World-Action Models (WAM). We further perform comprehensive ablations to validate key design choices of \textit{GigaBrain-W0}, including the effectiveness of robot-oriented pretraining, and  the role of Visual Feedforward Dynamics Modeling in coupling actions with pixels and providing denser supervision beyond action labels. We next describe the experimental setup and report detailed quantitative and qualitative comparisons.

% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/main_exp.pdf}
% \caption{Performance comparison between \textit{GigaBrain-0} and $\pi_0$ across six tasks on G1 and PiPER robot platforms, where (a) \texttt{Laundry Folding} and (b) \texttt{Paper Towel Preparation} are dexterous manipulation tasks; (c) \texttt{Juice Preparation} and (d) \texttt{Table Bussing} are long-horizon tasks; (e) \texttt{Boxes Moving} and (f) \texttt{Laundry Baskets Moving} are mobile manipulation tasks.}
% \label{fig:main_exp}
% \end{figure}


\subsection{Real World Manipulation Experiment}


\textbf{Experiment Setup.}
We evaluate \textit{GigaBrain-0} on two dexterous manipulation tasks, \texttt{laundry folding} and \texttt{paper towel preparation}. For \texttt{laundry folding}, we deploy the model on the G1 robot platform and fine-tune it using 300 human-collected demonstration trajectories, the training is conducted with a batch size of 128 for 40K steps. For \texttt{paper towel preparation}, we use 100 demonstrations from PiPER arms, and the training is conducted with a batch size of 128 for 20K steps.
We compare \textit{GigaBrain-0} against $\pi_0$~\citep{pi0}, which is implemented using the official open-source code, and fine-tuned with the same training config for fair comparison.

% We compare \textit{GigaBrain-0} against three established baselines: $\pi_0$~\citep{pi0}, $\pi_{0.5}$~\citep{pi05}, and WALL-OSS~\citep{walloss}, all implemented using their official open-source code, and fine-tuned with the same data for fair comparison.

% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/piper_laundry.pdf}
% \caption{Deployment of \textit{GigaBrain-0} on the G1 humanoid robot for real-world \texttt{laundry folding}.}
% \label{fig:laundry_demo}
% \end{figure}

% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/towel_prepare.pdf}
% \caption{Deployment of \textit{GigaBrain-0} on the PiPER arms for real-world \texttt{paper towel preparation}.}
% \label{fig:papertowel_demo}
% \end{figure}


\textbf{Experiment Results.}
As shown in Fig.~\ref{fig:main_exp}(a--b), \textit{GigaBrain-0} consistently achieves the highest task success rate across both tasks, surpassing $\pi_{0}$ by 30\% and 10\% in each case. Its integration of depth sensing enhances spatial awareness, enabling precise coordination in contact-rich scenarios. Qualitatively, as illustrated in Fig.~\ref{fig:laundry_demo} and Fig.~\ref{fig:papertowel_demo}, \textit{GigaBrain-0} robustly executes complex, dexterous workflows: for laundry, it performs synchronized dual-gripper grasping, accurate folding, and final alignment; for paper towels, it tears off excess material, rolls the towel with controlled tension, and precisely applies adhesive labels. These results highlight \textit{GigaBrain-0}'s superior dexterous manipulation capability and generalization in real-world, unstructured settings.



% \subsection{Long-horizon Experiment}


% \textbf{Experiment Setup.}
% We evaluate \textit{GigaBrain-0} on two long-horizon manipulation tasks: \texttt{table bussing} and \texttt{juice preparation}. For \texttt{table bussing}, we deploy the model on the dual-arm PiPER robot platform and fine-tune it using 100 human-collected demonstration trajectories, and the training is conducted with a batch size of 128 for 20K steps. For \texttt{juice preparation}, we utilize the AgiBot G1 robot with 489 demonstrations, and the training is conducted with a batch size of 128 for 35K steps. We compare \textit{GigaBrain-0} against $\pi_{0}$~\citep{pi0}, which is implemented using the official open-source code, and fine-tuned with the same training config to ensure a fair comparison.

% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/table_buss.pdf}
% \caption{Deployment of \textit{GigaBrain-0} on PiPER arms for real-world \texttt{table bussing}.}
% \label{fig:table_demo}
% \end{figure}

% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/juice.pdf}
% \caption{Deployment of \textit{GigaBrain-0} on G1 humanoid robot for real-world \texttt{juice preparation}.}
% \label{fig:juice_demo}
% \end{figure}


% \textbf{Experiment Results.}
% As shown in Fig.~\ref{fig:main_exp}(c--d), \textit{GigaBrain-0} consistently achieves the highest task success rate across both long-horizon tasks. Its integration of embodied Chain-of-Thought (CoT) reasoning enables fine-grained, temporally ordered planning—critical for complex multi-step execution. Qualitative results in Fig.~\ref{fig:table_demo} and Fig.~\ref{fig:juice_demo} further demonstrate \textit{GigaBrain-0}'s robustness: in \texttt{table bussing}, it first detaches bowls from plates, then sequentially places plates followed by bowls into the collection bin. In \texttt{juice preparation}, it scoops powdered mix with a spoon, dispenses water from the dispenser, and finally stirs the mixture to completion. These results highlight \textit{GigaBrain-0}'s superior capacity for structured reasoning and reliable execution in long-horizon, real-world manipulation scenarios.


% \subsection{Mobile Manipulation Experiment}


% \textbf{Experiment Setup.}
% We evaluate \textit{GigaBrain-0} on two mobile manipulation tasks: \texttt{boxes moving} and \texttt{laundry baskets moving}. For \texttt{boxes moving}, we deploy the model on the AgiBot G1 robot platform and fine-tune it using 300 human-collected demonstration trajectories, and the training is conducted with a batch size of 128 for 30K steps. For \texttt{laundry baskets moving}, we utilize the dual-arm PiPER robot platform with 378 demonstrations, and the training is conducted with a batch size of 192 for 30K steps. We compare \textit{GigaBrain-0} against $\pi_0$~\citep{pi0}, which is implemented using the official open-source code, and fine-tuned with the same training config to ensure a fair comparison.

% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/box_move.pdf}
% \caption{Deployment of \textit{GigaBrain-0} on the G1 humanoid robot for real-world \texttt{paper towel preparation}.}
% \label{fig:boxes_demo}
% \end{figure}


% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/laundry_move.pdf}
% \caption{Deployment of \textit{GigaBrain-0} on the PiPER arms for real-world \texttt{laundry baskets moving}.}
% \label{fig:baskets_demo}
% \end{figure}


% \textbf{Experiment Results.}
% As shown in Fig.~\ref{fig:main_exp}(e--f), \textit{GigaBrain-0} achieves the highest success rate in both mobile manipulation tasks, surpassing $\pi_{0}$  by 10\% in each task. Its unified architecture, combining global navigation priors with local manipulation policies, enables seamless transitions between mobility and interaction. In \texttt{boxes moving}, \textit{GigaBrain-0} navigates around obstacles, identifies target boxes using semantic segmentation, grasps them with adaptive force control, and delivers them to designated zones. In \texttt{laundry baskets moving}, it locates partially occluded baskets, adjusts its base position for optimal reach, lifts baskets using compliant gripper control, and transports them across uneven terrain without spilling contents. Qualitative results in Fig.~\ref{fig:boxes_demo} and Fig.~\ref{fig:baskets_demo} further illustrate \textit{GigaBrain-0}'s robustness to environmental variability and its ability to recover from minor localization or grasping errors through real-time replanning.


% \begin{figure}[t]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/generalization_exp.png}
% \caption{Generalization performance of \textit{GigaBrain-0} under appearance, placement, and viewpoint shifts. The horizontal axis denotes the sampling probability $\alpha$  of world model-generated data used during training. }
% \label{fig:generalization_exp}
% \end{figure}


% \subsection{Manipulation Generalization Experiment}
% Diverse training data is crucial for the generalization of VLA models~\citep{shi2025diversity}. \textit{GigaBrain-0} leverages GigaWorld to generate diverse training data, which significantly enhances its robustness and generalization under variations in appearance, object placement, and camera viewpoint. Below, we present our experimental setup and analysis in detail.

% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/appearance_transfer.pdf}
% \caption{Illustration of the appearance generalization experiment on \texttt{laundry folding}: one white garment and nine items with varied colors and textures.}
% \label{fig:appearance}
% \end{figure}


% \textbf{Appearance Generalization.} We conduct appearance generalization experiments on the \texttt{laundry folding} task. Specifically, we perform post-training on \textit{GigaBrain-0} using a small set of real-world folding demonstrations, limited to only 50 trajectories of white garments collected on the physical robot. To enhance visual diversity, we combine this real data with trajectories generated by the GigaWorld Real2Real transfer model, which effectively transfers appearance attributes while preserving geometric and dynamic consistency (see Fig.~\ref{fig:real2real} for illustration).
% We then evaluate how the mixing ratio $\alpha$ (i.e., the probability of sampling generated data in each training batch) affects real-world success rates. The model is fine-tuned for 20k steps with a batch size of 128. For evaluation, we test on 10 distinct garments with diverse appearances, including the original white garments and 9 additional items with varied colors and textures (examples shown in Fig.~\ref{fig:appearance}). Each garment is folded five times, and success is measured per trial. 
% As shown in Fig.~\ref{fig:generalization_exp}(a), for a complex deformable manipulation task like garment folding, training exclusively on white garments leads to poor generalization to real-world garments with diverse textures and colors. However, incorporating appearance-transferred data significantly improves texture generalization. Notably, as the sampling probability $\alpha$ of generated data increases from 0 to 50\%, the success rate rises substantially, reaching nearly 70\%. Further increasing $\alpha$ to 75\% and 90\% yields additional gains, pushing the success rate above 80\%.


% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/placement.pdf}
% \caption{Illustration of the object placement generalization experiment on \texttt{table bussing}: one collected placement and nine novel object placements.}
% \label{fig:placement}
% \end{figure}



% \textbf{Placement Generalization.} We investigate generalization to novel object placements in the table bussing task. Our approach begins with post-training \textit{GigaBrain-0} on a small set of real-world demonstrations, only 50 trajectories collected under a single, fixed bowl configuration. To broaden the distribution of object positions during training, we supplement this limited real data with trajectories produced by the GigaWorld Sim2Real transfer model. This model not only introduces a wide variety of object placements but also enhances visual realism by adapting simulated appearances to better match real-world conditions (see Fig.~\ref{fig:sim2real}).
% We study the impact of the mixing ratio $\alpha$ on downstream performance. The policy is fine-tuned for 20k steps with a batch size of 128. During evaluation, we assess performance across 10 distinct placement layouts: the original fixed setup with 9 new configurations with diverse object placements (examples in Fig.~\ref{fig:placement}). Each layout is tested five times, and success is recorded per trial.
% Results in Fig.~\ref{fig:generalization_exp}(b) reveal that, for this long-horizon bussing task, models trained solely on fixed-placement data struggle to handle real-world variations in object layout. In contrast, blending in Sim2Real transferred data dramatically boosts generalization to unseen placements. As $\alpha$ increases from 0 to 75\%, the success rate climbs sharply, surpassing 90\%. This gain arises because the simulation provides abundant novel placement scenarios that teach the policy manipulation behaviors, while the Sim2Real transfer simultaneously mitigates the visual domain gap between simulation and real images.

% \textbf{Viewpoint Generalization.} We investigate generalization to novel camera viewpoints in the table bussing task. Begining by post-training \textit{GigaBrain-0} on a small set of 50 real-world demonstrations, all captured from a single, fixed camera viewpoint. To enrich viewpoint diversity during training, we augment this data with trajectories generated by the GigaWorld view transfer model, which effectively re-renders the originally collected demonstrations from a broad range of virtual camera angles while preserving task-relevant robot actions (see Fig.~\ref{fig:view_transfer}).
% We analyze how the mixing ratio $\alpha$ influences real-world performance. The policy is fine-tuned for 20k steps with a batch size of 128. For evaluation, we test on 9 distinct camera viewpoints: the original fixed view plus 8 additional, previously unseen viewpoints with varied positions and rotations (examples shown in Fig.~\ref{fig:view}). Each viewpoint is evaluated over five independent trials, with success judged per trial.
% As shown in Fig.~\ref{fig:generalization_exp}(c), when trained only on data from a single viewpoint, the policy exhibits significant performance degradation under novel viewing conditions. In contrast, incorporating view-transferred data substantially improves robustness to viewpoint shifts. As $\alpha$ increases from 0 to 90\%, the success rate rises sharply, exceeding 80\%. This improvement is attributed to two factors: (1) exposure to multi-view observations enables the policy to learn viewpoint-invariant visual representations, and (2) the GigaWorld view transfer model provides photorealistic, geometrically consistent renderings that closely approximate real-world visual input from arbitrary angles.

% \begin{figure}[htbp]
% \centering
% \captionsetup{type=figure, justification=justified, singlelinecheck=false}
% \includegraphics[width=1\linewidth]{images/view.pdf}
% \caption{Illustration of the camera viewpoint generalization experiment on \texttt{table bussing}: one collected viewpoint and eight novel camera viewpoints.}
% \label{fig:view}
% \end{figure}


\subsection{Inference Speed}
While existing WAS models demonstrate strong manipulation capability, they often incur substantial inference overhead, resulting in high end-to-end latency. Efficient on-device execution, however, is critical for real-time robotic applications that demand low latency, privacy, and autonomy. To this end, we conduct a systematic comparison of inference efficiency across several representative models.

As shown in Tab.~\ref{tab:time}, we compare \textit{GigaBrain-W0} against multiple baselines. We observe that some methods (e.g., Motus) require significantly higher compute (GFLOPs), which translates into substantially longer inference latency. Importantly, long inference latency can materially degrade closed-loop performance in the real world: for deformable-object manipulation tasks such as laundry folding, the scene can evolve rapidly and contact dynamics are highly sensitive. Insufficient control frequency leads to misalignment between actions and observations, which in turn increases the likelihood of failed grasps, slippage, and error accumulation.

Moreover, these approaches often come with a larger memory footprint (both RAM and VRAM), further constraining deployment and scalability on resource-limited platforms (e.g., edge devices or mobile robot compute modules).

In contrast, \textit{GigaBrain-W0} achieves lower compute and memory consumption while maintaining competitive performance, and it delivers faster inference. This improves responsiveness and stability in closed-loop control and makes \textit{GigaBrain-W0} a more practical choice for real-time, on-device deployment.

\begin{table}[htbp]
\centering
\caption{Model comparison between \textit{GigaBrain-0-Small} and $\pi_0$ on the Orin platform.}
\label{tab:time}
\begin{tabular}{lcccccc}
\toprule
Model & FLOPs & Parameters & Inference VRAM & Inference Latency & Success Rate \\
      & (GFLOPs) & (B/M) & (GB) & (seconds) & \\
\midrule
$\pi_0$ & 4400 & 3.2\,B & 17.5 & 1.28 & 80\% \\
% \textit{GigaBrain-0-Small} & 840 & 402\,M & 1.9 & 0.13 &  80\% \\
$\pi_0$ & 4400 & 3.2\,B & 17.5 & 1.28 & 80\% \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Manipulation Generalization Experiment}
We further evaluate the generalization capability of different WAM. In particular, we focus on two practically important generalization axes: appearance generalization and placement generalization.

\textbf{Appearance Generalization.} We conduct appearance generalization experiments on the \texttt{fold\_cloth} task. Concretely, we fine-tune all WMS models using a small set of real-robot demonstrations collected on a single garment type: \textbf{50 trajectories on a white cloth only}. At evaluation time, we test on \textbf{10 garments} with diverse appearances, including the original white cloth and \textbf{9 unseen cloths} with different colors and textures (examples in Fig.~\ref{fig:appearance_generalization}, corresponding to your Fig.~18). Each garment is evaluated for 5 independent trials, and we record success on a per-trial basis.
As shown in Tab.~\ref{tab:generalization}, \textit{GigaBrain-W0} achieves a clearly higher success rate, indicating stronger robustness to appearance shifts under limited real-world supervision.

\paragraph{Placement Generalization.} We additionally examine placement generalization on the remaining tasks (e.g., tabletop manipulation). During training, we fine-tune each WMS model with \textbf{50 real-world demonstration trajectories} collected under a \textbf{single fixed object/bowl placement}. During evaluation, we test on \textbf{10 layouts} in total: the original fixed layout and \textbf{9 novel layouts} with different object placements (examples in Fig.~\ref{fig:placement_generalization}, corresponding to your Fig.~19). We repeat each layout for 5 trials and record success for each trial.
The results in Fig.~\ref{fig:long_horizon_generalization} (your Fig.~17(b)) suggest that, for long-horizon tasks such as table bussing, models trained only on fixed-placement demonstrations struggle to cope with real-world layout variations. In contrast, \textit{GigaBrain-W0} exhibits stronger placement generalization across all evaluated tasks (Tab.~\ref{tab:generalization}), demonstrating improved robustness to distribution shifts in object arrangements.

\begin{table}[t]
\centering
\caption{Success rates (\%) on appearance and placement generalization benchmarks.}
\label{tab:generalization}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Methods} &
\multicolumn{1}{c}{\textbf{Appearance Gen.}} &
\multicolumn{3}{c}{\textbf{Placement Gen.}} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-5}
& \texttt{fold\_cloth} & \texttt{pour\_fried} & \texttt{scan\_qr} & \texttt{sweep\_the\_trash} \\
\midrule
Motus      & xx.x & xx.x & xx.x & xx.x \\
Baseline-A & xx.x & xx.x & xx.x & xx.x \\
Baseline-B & xx.x & xx.x & xx.x & xx.x \\
\textit{GigaBrain-W0} & \textbf{xx.x} & \textbf{xx.x} & \textbf{xx.x} & \textbf{xx.x} \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Ablation Study}
We conduct ablation studies in real-world settings to validate the key design choices of \textit{GigaBrain-W0}. Unless otherwise specified, all ablations are fine-tuned with the same data budget and optimization hyperparameters as the main experiments, and are evaluated using identical protocols.


\begin{table}[t]
\centering
\caption{Ablation on multi-stage pre-training.}
\label{tab:ablation_stage}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lccc}
\toprule
Stage~1 & Stage~2 & Stage~3 & SR (\%) \\
\midrule
 &  & \checkmark & xx.x \\
\checkmark &  & \checkmark & xx.x \\
\checkmark & \checkmark & \checkmark & \textbf{xx.x} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{Ablation on pretraining data sources (remove-one-source).}
\label{tab:ablation_data}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lcc}
\toprule
Setting & Removed source & SR (\%) \\
\midrule
Full & -- & \textbf{xx.x} \\
(a) w/o Task-Agnostic Data & Stage~1 (\texttt{img+txt}) & xx.x \\
(b) w/o Web Data & Stage~1 (\texttt{img+txt}) & xx.x \\
(c) w/o Multi-Robot Traj. & Stage~1 (\texttt{img+txt}) & xx.x \\
(d) w/o Egocentric Human Videos & Stage~2 (\texttt{img+txt+act}) & xx.x \\
(e) w/o World Model Generation Data & Stage~2 (\texttt{img+txt+act}) & xx.x \\
\bottomrule
\end{tabular}
\end{table}


\textbf{Impact of multi-stage pretraining.}
We first study how each training stage contributes to downstream manipulation performance. Starting from the same initialization, we progressively enable Stage~1 (robot-oriented video pretraining), Stage~2 (action-conditioned pretraining with unified tokens), and Stage~3 (target-robot fine-tuning). Tab.~\ref{tab:ablation_stage} reports success rates under each configuration.

We observe a monotonic improvement as additional stages are included. Stage~1 provides a strong spatiotemporal representation prior in robotic scenes, Stage~2 aligns the backbone with action-conditioned prediction and reduces ambiguity in multi-modal futures.


\textbf{Effect of pretraining data sources.}
We next investigate which pretraining data sources are most critical for WAM performance. Starting from the full training recipe, we perform a remove-one-source ablation: we drop one data category at a time, keep all other settings fixed, and re-run fine-tuning. Specifically, we consider Stage~1 data (\texttt{images+text}: task-agnostic robotic data, synthetic data, web data, and multi-robot task trajectories) and Stage~2 data (\texttt{images+text+action}: egocentric human videos, synthetic data, and world-model-generated data).
Tab.~\ref{tab:ablation_data} reports the results. We find that action-rich sources---in particular \textit{egocentric human videos} and \textit{world-model-generated data}---contribute disproportionately to success. Moreover, simulation-based synthetic data provides complementary coverage of rare interactions and corner-case configurations that are difficult to collect in the real world. Intuitively, these sources expand training diversity over contact-rich behaviors and long-tail object configurations, and they promote learning action-relevant visual features that transfer better under distribution shift.

\begin{table}[t]
\centering
\caption{Ablation on pretraining data sources (remove-one-source).}
\label{tab:ablation_data}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lcc}
\toprule
Setting & Removed source & SR (\%) \\
\midrule
Full & -- & \textbf{xx.x} \\
(a) w/o Task-Agnostic Data & Stage~1 (\texttt{img+txt}) & xx.x \\
(b) w/o Web Data & Stage~1 (\texttt{img+txt}) & xx.x \\
(c) w/o Multi-Robot Traj. & Stage~1 (\texttt{img+txt}) & xx.x \\
(d) w/o Egocentric Human Videos & Stage~2 (\texttt{img+txt+act}) & xx.x \\
(e) w/o World Model Generation Data & Stage~2 (\texttt{img+txt+act}) & xx.x \\
\bottomrule
\end{tabular}
\end{table}



\textbf{Role of Visual Feedforward Dynamics Modeling.} A core component of \textit{GigaBrain-W0} is \textit{Visual Feedforward Dynamics Modeling}, which couples actions with pixel-level consequences and provides dense supervision beyond action labels. To isolate its effect, we compare the following variants (Tab.~\ref{tab:ablation_vfd}):

\begin{itemize}
    \item \textbf{Action-only}: removes the dynamics objective and trains only with action supervision (no future video prediction).
    \item \textbf{Joint prediction w/o causal mask}: predicts both action and future video but removes the blockwise causal mask, allowing information leakage that weakens the intended ``history $\rightarrow$ action'' constraint.
    \item \textbf{Ours (VFD + causal masking)}: the full model, where action tokens are predicted from history only, while video tokens are predicted from history + (teacher-forced) actions.
\end{itemize}

We observe that action-only training is consistently weaker, especially on contact-rich and deformable manipulation, confirming that sparse action labels are insufficient to learn robust, action-relevant representations. Training joint action/video \emph{without} causal masking does not reliably improve performance and can even degrade it, suggesting that improper information flow harms the action inference pathway. In contrast, the full \textit{GigaBrain-W0} formulation yields the best results, validating that dynamics prediction is most beneficial when it is \emph{explicitly conditioned on actions} and \emph{properly causally structured}.

\begin{table}[t]
\centering
\caption{Ablation on Visual Feedforward Dynamics Modeling (VFD).}
\label{tab:ablation_vfd}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lccc}
\toprule
Method & Predict future video & Causal mask & SR (\%) \\
\midrule
Action-only (IL) &  &  & xx.x \\
Joint w/o mask & \checkmark &  & xx.x \\
Ours (VFD) & \checkmark & \checkmark & \textbf{xx.x} \\
\bottomrule
\end{tabular}
\end{table}


\textbf{Multi-view fusion design.}
Finally, we study how to incorporate multi-view observations into pretrained video generation models. Our default design concatenates synchronized views along the width dimension (\emph{view concatenation}), which preserves per-view spatial structure while allowing a single backbone to model cross-view correspondences. We compare against two alternative fusion strategies (Tab.~\ref{tab:ablation_multiview}): (i) \textbf{Single-view}, where each view is processed independently and no concatenation is performed (we report the front view); (ii) \textbf{Motus-style prioritized concatenation}, which concatenates views with an imbalanced allocation of tokens that prioritizes the front view; and (iii) \textbf{Equal-weight concatenation} (ours), which assigns equal importance to all views and concatenates them uniformly (see Fig.~\ref{fig:multiview_fusion}, corresponding to your Fig.~12).

In Tab.~\ref{tab:ablation_multiview}, we report both success rate and the resulting number of input tokens. We find that \textbf{equal-weight concatenation} achieves the best performance when the token budget is affordable. We attribute this gain to two factors. First, the single-view baseline ignores cross-view consistency, making it more brittle under occlusions and viewpoint-specific ambiguities. Second, prioritized concatenation over-emphasizes the front camera and can under-utilize informative close-up views. In practice, the left/right wrist cameras provide fine-grained contact and local geometry cues (e.g., grasp points and wrinkles) that are difficult or impossible to infer reliably from the front view alone; treating these views as first-class inputs improves action grounding and robustness.

\begin{table}[t]
\centering
\caption{Ablation on multi-view input fusion. We report the resulting number of input tokens and success rate (SR) for different fusion strategies.}
\label{tab:ablation_multiview}
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lcc}
\toprule
Fusion strategy & Tokens & SR (\%) \\
\midrule
Single-view & xx & xx.x \\
Motus-style prioritized concat & xx & xx.x \\
Equal-weight view concat (ours) & xx & \textbf{xx.x} \\
\bottomrule
\end{tabular}
\end{table}


% \textbf{多阶段预训练对成功率的影响}在预训练部分我们探究了xxxx ，我们分别探讨第一阶段和第二阶段预训练的有效性。as shown in xxx 我们

% 第一阶段 第二阶段  第三阶段    SR

% \textbf{预训练数据对成功率的影响}
% 我们在与训练阶段主要使用了xxxx xxxx的数据，我们分别探究其对xxx的作用
% Task-Agnostic Data; Synthetic Data; Web Data; Multi-Robot Task Tra-
% jectory Data
% 2 images + text + action Egocentric Human Videos; Synthetic Data; World Model Generation
% Data
% 我们发现xxxx 尤其是 action Egocentric Human Videos; World Model Generation
% Data非常重要 因为xxxx


% \textbf{使用Visual Feedforward Dynamics Modeling作为reasong分支对成功率的影响}
% 在Gigabrain-w0中，我们使用xxx作为xxx分支而不是xxx。我们对比了几种模型，第一种只使用action作为监督
% ，不预测未来视频 第二种不使用casual mask同时出视频和动作 第三种为GigaBrain-w0 as shown xxx
% \textbf{多视角输入的组合方式 对成功率的影响}


==> sections/GigaBrain_Model.tex <==
\section{GigaBrain-WA0 Model}

% \begin{equation}
% \mathcal{L}=\ell\big(p_\theta(a_{t:t+p-1}\mid o_{\le t}, s_t, l),\, a_{t:t+p-1}\big),
% \end{equation}

\subsection{Problem Statement \& Approach Overview}
We formulate robotic manipulation as a sequential decision-making task. At each time step $t$, the robot receives multi-view RGB observations $o_t=\{o_t^v\}_{v\in S}$ with $S=\{\text{left},\text{front},\text{right}\}$, a natural-language instruction $l$, and the proprioceptive state $s_t$. Conditioned on these inputs, the policy predicts an action chunk of length $p$, $a_{t:t+p-1}=(a_t,a_{t+1},\ldots,a_{t+p-1})$, where $p$ denotes the number of actions in the chunk.

\textbf{Vision-Language-Action Policies.} Most existing vision-language-action (VLA) policies are trained via imitation learning to model and sample an action chunk conditioned on the observation history, the robot state, and a language instruction:
\begin{equation}
a_{t:t+p-1} \sim p_\Theta(\,\cdot \mid o_{\le t},\, s_t,\, l\,).
\end{equation}
Here, $o_{\le t}$ denotes the observation history up to time $t$, $s_t$ is the robot state at time $t$, and $l$ is the language input. The distribution $p_\Theta(\,\cdot \mid o_{\le t}, s_t, l)$ parameterizes the policy over the next $p$ actions. In this paradigm, learning is driven solely by action supervision from demonstrations, without any explicit supervision on the predicted consequences in the observation space.


% Most existing vision-language-action (VLA) policies are trained via imitation learning  to learns to sample an action chunk conditioned on history, state, and language:
% \begin{equation}
% a_{t:t+p-1} \sim p_\Theta(\,\cdot \mid o_{\le t},\, s_t,\, l\,).
% \end{equation}
% where $o_{\le t}$ denotes the observation history up to time $t$, $p_\theta(a_{t:t+p-1}\mid o_{\le t}, s_t, l)$ is the learned action-chunk distribution, and $\ell(\cdot)$ is a standard action loss. Therefore, supervision is provided only through the action labels.

\textbf{Our Approach.}  Unlike approaches that only model an action distribution, we adopt a world-modeling perspective that additionally learns how visual observations evolve under an executed action chunk. We implement our method as a single unified model $g_\Theta$ that parameterizes two complementary conditional distributions. For action modeling, anchored by demonstrations, the model learns to sample an action chunk conditioned on the observation history, robot state, and language:
\begin{equation}
a_{t:t+p-1} \sim g_\Theta(\,\cdot \mid o_{\le t},\, s_t,\, l\,).
\label{2}
\end{equation}
For visual feedforward dynamics modeling, given the same context and the executed action chunk, the model learns to sample a future observation sequence that captures the evolution of visual observations:
\begin{equation}
o_{t+\Delta,\, t+2\Delta,\, \ldots,\, t+K\Delta}
\sim g_\Theta\!\big(\,\cdot \mid o_{\le t},\, s_t,\, l,\, a_{t:t+p-1}\big),
\qquad \Delta \ge 1.
\label{1}
\end{equation}
where $\Delta$ denotes the temporal stride between predicted observations, $K$ is the number of predicted observation steps. Together, these two learned conditionals couple decision-making with consequence prediction, yielding representations that are both behaviorally grounded and visually predictive. Importantly, action selection at inference can rely on the learned action-chunk distribution alone, treating visual forecasting primarily as a training-time visual reasoning signal.


\subsection{GigaBrain-WA0: Architecture }
We build \textit{GigaBrain-WA0} by adapting a 5B-parameter diffusion Transformer. We then further pretrain it with an action-centric objective to obtain a world-action model tailored to robotic manipulation. Furthermore, we concatenate multi-view inputs to enable joint reasoning over multi-view observations while encouraging cross-view consistency. Finally, to unify action modeling and visual feedforward dynamics modeling within a single model, we employ a causal masking scheme that places observation and action tokens in a single sequence and enforces the desired conditional factorization.

\textbf{Action-centered pretraining.}
We perform a two-stage action-centered pretraining to better align the backbone with our approach modeling.
In Stage~1, we pretrain on robot datasets to generate future video conditioned on text and the first frame based in the Wan2.2~\cite{wan}.
In Stage~2, we continue training from Stage~1 to further match our setting.
We use the resulting weights as the pretraining of \textit{GigaBrain-WA0}. 

\textbf{Multi-view conditioning by view concatenation.} 
To enable multi-view generation without modifying the backbone while encouraging cross-view consistency, we concatenate the three views along the width dimension:
\begin{equation}
o_t^{\text{concat}} = [\,o_t^{\text{left}};\,o_t^{\text{front}};\,o_t^{\text{right}}\,].
\label{concat}
\end{equation}
This representation preserves the spatial structure of each view within a shared coordinate frame and assigns comparable importance to all views, facilitating cross-view consistency across the concatenated panorama.

\textbf{State and action projector.}
We map proprioceptive states and actions into the pretrained model's hidden dimension via learnable linear projections. The resulting embeddings are appended to the visual token sequence as additional tokens, enabling unified spatiotemporal reasoning over pixels, states, and actions.

\textbf{Shared Transformer blocks.}
Unlike MoE-based designs, we process all token types with a single shared stack of Transformer blocks.
In particular, visual and action tokens share the same query/key/value projection matrices at every layer, which tightly couples action tokens with visual evidence while preserving the computational profile of the pretrained backbone.
Meanwhile, we use different positional encodings for different token types to respect their underlying structures: visual tokens adopt a 2D positional encoding over the image grid, whereas proprioceptive state/action tokens use a 1D temporal positional encoding along the sequence dimension.


% \textbf{Causally-masked joint attention for video--action modeling.}
% To unify action generation and visual dynamics modeling in a single diffusion Transformer, we place all modalities into one token sequence and apply a causal attention mask to control information flow.
% Concretely, we use the concatenated multi-view observation $o_t^{\text{concat}}$  as visual input, and append the projected proprioceptive state and action embeddings as additional tokens.
% The mask allows each action token to attend to the instruction, proprioception, and the first-frame visual tokens, while blocking access to future visual tokens. Meanwhile, video tokens are allowed to attend to state/action tokens to incorporate control context, enabling coherent joint training; at inference time, we can drop the video tokens and decode only actions for efficiency (Sec.~X).

\textbf{Causally-masked joint attention for video--action modeling.}
To unify action generation and visual dynamics modeling within a single diffusion Transformer, we place all modalities into one token sequence and apply a causal attention mask to regulate information flow.
Concretely, we use the concatenated multi-view observation $o_t^{\text{concat}}$ as the visual input, and append the projected proprioceptive states and action embeddings as additional tokens.
The mask allows each action token to attend to proprioceptive tokens and the first-frame visual tokens, while preventing access to future visual tokens.
Meanwhile, video tokens are allowed to attend to all tokens, enabling coherent joint training.
At inference time, for efficiency, we can drop the video tokens and decode only actions, since action prediction does not depend on future visual tokens.


% To jointly model visual dynamics and action generation in a single diffusion Transformer, we apply a causal attention mask to enforce the desired information flow.
% Specifically, action tokens attend to the instruction and proprioception, and are grounded by attending to the first-frame visual tokens, while being prevented from attending to future action tokens; meanwhile, video tokens may attend to state/action tokens to incorporate control-relevant context.
% This masking scheme enables coherent joint modeling during training and allows us to remove the video-related branch at inference time for efficiency (see Sec.~X).



\subsection{GigaBrain-WA0: Training}
In this section, we describe both the pretraining and post-training processes. For post-training, we detail the training inputs, our causal masking design, and the joint objectives that couple action modeling with feedforward visual dynamics modeling. For pretraining, we present the overall pretraining design and the datasets used in each stage.

\subsubsection{Post-training}
\label{Post-training}
\noindent\textbf{Training input.}
Each training sample is a short manipulation segment, consisting of a natural-language instruction $l$, synchronized multi-view RGB observations $o_t^{concat}$, proprioceptive states $s_t$, and an action sequence $a_{t:t+p-1}$. 
As shown in Eq.~\ref{1}, dense future-frame prediction is often redundant due to high temporal correlations. Therefore, we predict future observations $\{\,o^{concat}_{t+k\Delta}\,\}_{k=1}^{K}$ at a fixed stride, i.e., one frame every $\Delta$ steps along the action horizon.  Then, we encode both the current and predicted future observations, $o_t^{concat}$ and $\{\,o^{concat}_{t+k\Delta}\,\}_{k=1}^{K}$, with the same VAE and tokenize the resulting latents into spatiotemporal visual tokens $T_{obs}$ and $T_{future}$. 
In parallel, we embed proprioceptive states and actions into state tokens $T_s$ and action tokens $T_a$, respectively, and obtain the instruction token sequence $T_{text}$ by encoding $l$ with a pretrained language encoder.


\noindent\textbf{Causal masking design.}
As shown in Eq.~\ref{2} and Eq.~\ref{1}, our goal is to simultaneously perform \emph{action prediction} and \emph{visual feedforward dynamics modeling}, where future-frame reasoning is explicitly conditioned on the executed action chunk.
To realize both objectives within a single model, we linearize the interleaved video--action trajectory into one unified token sequence, so that a single Transformer can jointly couple decision-making with consequence prediction.
Notably, the language instruction is not included in this unified self-attention sequence; instead, $l$ is provided as an external conditioning signal  via  cross-attention, and thus does not participate in the causal ordering below. Concretely, at each step $t$, we concatenate all modalities into a single unified token sequence:
\begin{equation}
T_t
=
\big[\,T_s \,;\; T_{\mathrm{obs}} \,;\; T_a \,;\; T_{future}\,\big],
\label{tokens}
\end{equation}
We then impose a blockwise causal attention mask (Fig.~\ref{mask}) to enforce the desired information flow:
(i)  $T_s$ and $T_{obs}$ can attend to each other, but are blocked from attending to $T_a$ and $T_{future}$;
(ii) action tokens in $T_a$ can attend to the history tokens $\{T_s,\,T_{obs}\}$, but cannot attend to $T_{future}$;
(iii) future-video tokens in $T_{future}$ can attend to $\{T_s,\,T_{obs},\,T_a\}$, enabling feedforward dynamics prediction conditioned on the executed action chunk.
This masking scheme prevents leakage from predicted futures into action generation, while allowing future-frame prediction to leverage both observations and actions, consistent with Eq.~\ref{2} and Eq.~\ref{1}.

\noindent\textbf{Training objective.}
We use flow matching to jointly optimize action prediction and visual feedforward dynamics modeling.
For either modality $x$ (action tokens or future video tokens), we sample a flow time $s\sim\mathcal{U}(0,1)$ and noise $\epsilon\sim\mathcal{N}(0,I)$, and construct the interpolated noised variable
\begin{equation}
x^{(s)}=(1-s)\epsilon+s x,
\end{equation}
with target velocity
\begin{equation}
\dot{x}^{(s)}=x-\epsilon.
\end{equation}

Let $z_{\mathrm{future}}$ denote the VAE latents corresponding to the future observation tokens $T_{\mathrm{future}}$. We train the model to predict the velocity field of future latents conditioned on history and the executed action chunk:
\begin{equation}
\mathcal{L}_{\mathrm{video}}
=
\mathbb{E}_{s,\epsilon}
\Big[
\big\|
g_\Theta\!\big(z_{\mathrm{future}}^{(s)},\, s \mid T_s,\,T_{\mathrm{obs}},\,T_a,\,T_{\mathrm{text}}\big)
-
\dot{z}_{\mathrm{future}}^{(s)}
\big\|^2
\Big].
\end{equation}

Similarly, letting $a$ denote the action-token representation for the action chunk $T_a$, we optimize an action flow-matching objective conditioned on history:
\begin{equation}
\mathcal{L}_{\mathrm{action}}
=
\mathbb{E}_{s,\epsilon}
\Big[
\big\|
g_\Theta\!\big(a^{(s)},\, s \mid T_s,\,T_{\mathrm{obs}},\,T_{\mathrm{text}}\big)
-
\dot{a}^{(s)}
\big\|^2
\Big].
\end{equation}

The overall training objective is
\begin{equation}
\mathcal{L}_{\mathrm{all}}
=
\mathcal{L}_{\mathrm{video}}
+
\mathcal{L}_{\mathrm{action}}.
\end{equation}


\subsubsection{Pre-training}
\noindent\textbf{Pre-training Process.}
We pre-train \textit{GigaBrain-WA0} in two structured stages to progressively inject robotic physical-interaction priors from diverse datasets. Each stage targets a key challenge: (i) adapting a general video generator to robot-centric multi-view observations, and (ii) aligning the representation with action-conditioned prediction required by our world-action formulation. The resulting weights are then used to initialize post-training for target-robot specialization (Sec.~\ref{Post-training}).

In Stage~1, we initialize from a video generation model pre-trained on large-scale Internet video data and further pre-train it on robot-scene multi-view data by concatenating views as in Eq.~\ref{concat}. This stage preserves the model's generic spatiotemporal modeling capability while adapting it to robotic environments, encouraging geometric consistency across viewpoints, robustness to viewpoint-induced appearance changes, and faithful modeling of object interaction dynamics.

In Stage~2, starting from the Stage~1 checkpoint, we explicitly introduce state and action conditioning to align the model with the downstream objectives of \textit{GigaBrain-WA0}. Concretely, we project proprioceptive states and actions into the same hidden dimension as the video tokens, concatenate them with the video tokens into a unified sequence (analogous to Eq.~\ref{tokens}), and supervise action-conditioned future video generation. This design addresses a fundamental ambiguity in manipulation: the first-frame observation alone often does not uniquely determine future evolution. For example, in bimanual tasks, visually similar starting states can lead to distinct trajectories depending on whether the left or right arm moves first. Injecting action signals is therefore essential for learning a consistent observation--action--future mapping and for reducing ambiguity.

% \noindent After pre-training, we fine-tune the model on target-robot data for specialization, and use the resulting weights to initialize post-training, as described in Sec.~\ref{Post-training}.

% GigaBrain-W0 is pre-trained in two structured stages, progressively integrating robot physical-interaction priors from diverse datasets to pretrain a pretrained model  Each stage addresses a key challenge: cross-domain representation learning, action-conditioned alignment.zuihou 使用这个预训练权重for post training for target-robot specialization.

% In Stage~1, we start from a video generation model pre-trained on large-scale video data and further pre-train it on multi-view data collected in robotic scenes by concating these views in Eq.~\ref{concat}. This stage aims to preserve the model's general spatiotemporal modeling capability while adapting it to robotic environments by capturing geometric consistency, viewpoint-induced variations, and the spatiotemporal dynamics of object interactions.

% In Stage~2, we explicitly introduce action conditioning during training to align the model with the subsequent training objectives of GigaBrain-W0. Concretely, we map the state token and action token to the same dimensionality as the video token, concatenate them with the video tokens into a unified token sequence as similar as Eq.~\ref{tokens}, and supervise the resulting video generation. This design is motivated by the fact that, in robotic manipulation, the first-frame observation often does not uniquely determine the future evolution of the scene. For example, in bimanual manipulation, trajectories with highly similar observations may correspond to different action strategies (e.g., moving the left arm first versus the right arm first). Therefore, injecting action signals is essential for learning a consistent observation--action--future mapping and for reducing ambiguity.

% After pretraining, we specialize the model to the target robot by fine-tuning on target-robot data, completing the final training, as shown in Sec.~\ref{Post-training}

\noindent\textbf{Pre-training Data.}
To make pre-training maximally beneficial for the subsequent post-training and to improve generalization in manipulation, we curate datasets with increasing modality completeness and organize them into two groups by modality composition: language + images and language + images + actions. These two groups directly correspond to our two-stage pre-training recipe: Stage~1 focuses on learning general robot-scene representations from vision--language data, while Stage~2 introduces action signals to enable action-conditioned modeling and better align the backbone with Eq.~\ref{tokens} and our world-action objectives.


\begin{table*}[t]
\centering
\caption{Data modalities and sources used in the two-stage pre-training.}
\label{tab:training_data}
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabularx}{\textwidth}{c l X}
\toprule
\textbf{Stage} & \textbf{Data modalities} & \textbf{Data sources} \\
\midrule
1 & images + language &
Task-Agnostic Data; Synthetic Data; Web Data; Multi-Robot Task Trajectory Data \\
2 & images + language + actions &
Egocentric Human Data; Synthetic Data; World Model Generation Data \\
\bottomrule
\end{tabularx}
\end{table*}

As summarized in Table~\ref{tab:training_data}, Stage~1 primarily leverages vision--language data to adapt the pretrained video generator to robot scenes, while Stage~2 adds action supervision to learn an observation--action--future mapping that is consistent with downstream training.

Specifically, the Egocentric Human Data are supported by GigaWorld~\cite{gigaworld0}, which performs egocentric human video transfer by transforming first-person human hand motions into robot manipulation scenarios, effectively converting human demonstrations into robot-executable trajectories and expanding coverage for action-conditioned learning.
Meanwhile, the World Model Generation Data are also constructed with GigaWorld~\cite{gigaworld0} and include two complementary augmentations: (i) view transfer, which re-renders captured trajectories from diverse viewpoints to enrich perspective variations and encourage geometric consistency; and (ii) real-to-real appearance transfer, which generates diverse yet physically consistent changes in texture, color, lighting, and material properties, improving robustness to real-world distribution shifts.





% \textbf{
% 由于视频帧在时间维度上存在显著的冗余，这导致训练效率低下(2，我们对action chunk期间的动作进行一定的下采样因子为x来稀疏化视频序列，在减少视觉 token 数量的同时提升效率 [5]。，使得视频 token 与动作 token 的数量保持平衡


% \textbf{
% As Visual Feedforward Dynamics Modeling is a process for reasoning 动作是否合理， 同时这个过程以预测action为条件，therfore 我们可以将观察 动作 视频序列排列为单一的统一序列。 具体而言 我们的token排序为 
% Token_{state} Token_{obs} Token_{action} Token_{video} 
% 同时设置mask如Fig.~{ref1}, 动作部分只能干查到观察的历史状态 ，视频部分xxxx。这使得xxxxx

% \textbf{Training Objective}. We jointly optimize both video and action using flow matching with the noisy history augmentation
% described above. For video tokens zt, the dynamics loss supervises velocity field prediction conditioned on (potentially
% noisy) history



\subsection{GigaBrain-WA0: Inference}
At inference time, our goal is to generate actions with low latency under long-horizon, partially observed manipulation. Directly running the unified video--action diffusion Transformer would require sampling the future video-token stream at every control step, which is costly because video tokens are typically much longer than state/action tokens. Moreover, predicting future frames is not necessary for executing the policy. We therefore perform \emph{action-only decoding}, which retains the same backbone and tokenization as training while avoiding video generation overhead.

We keep the same conditioning pipeline for language, observations, and proprioception. At each control step $t$, we first form the context from the instruction, the current proprioceptive state, and the multi-view observation (concatenated as in Eq.~\ref{concat}):
\begin{equation}
c_t=\big(T_{\mathrm{text}},\ T_s,\ T_{\mathrm{obs}}\big).
\end{equation}
We then sample only the action chunk tokens $T_a$ from the learned action flow model conditioned on $c_t$, without instantiating any future video tokens. Concretely, we initialize $a^{(0)}\sim \mathcal{N}(0,I)$ and integrate the learned velocity field from $s=0$ to $s=1$:
\begin{equation}
\frac{d a^{(s)}}{d s}=g_\Theta\!\big(a^{(s)},\, s \mid c_t\big),\qquad s\in[0,1],
\end{equation}
obtaining $a^{(1)}$, which is then decoded to the continuous action chunk$\hat{a}_{t:t+p-1}$. Finally, we execute the action, observe the new state and images, and repeat the above procedure at the next control step. This inference procedure yields low-latency control by eliminating the need to sample future video tokens, while still benefiting from the dynamics-aware representations learned during joint training.


% At inference time, our goal is to generate actions with low latency under long-horizon, partially observed manipulation. A straightforward use of our unified video--action diffusion Transformer would require carrying the \emph{video token} stream at every step. However, video tokens are typically much longer than action/state tokens, which substantially increases sequence length, memory footprint, and sampling cost. Moreover, generating future frames is not required for executing the policy. We therefore adopt an \emph{action-only decoding} procedure that preserves the benefits of dynamics-aware training while avoiding video generation overhead.

% We keep the same backbone and tokenization used in training, but we \emph{do not instantiate nor sample} the future video tokens $V_{t\rightarrow}$ at test time. Concretely, at each control step $t$ we form the conditioning context
% \[
% c_t = \big(\texttt{Token}_{\text{lang}}(l),\ \texttt{Token}_{\text{state}}(s_{\le t}),\ \texttt{Token}_{\text{obs}}(o_{\le t})\big),
% \]
% and sample only the action tokens $A_t$ from the learned action flow/diffusion model:
% \[
% A_t \sim p_\Theta(A_t \mid c_t).
% \]
% Because the model was trained with a blockwise causal mask where action tokens never attend to future video tokens, removing $V_{t\rightarrow}$ at inference is \emph{architecturally consistent}: the action generation pathway is fully defined by language and history tokens. This yields a substantial reduction in compute and memory by eliminating the long video-token stream, enabling faster control loops.



% % 在推理阶段 由于xxx  我们不需要对视频部分，相较于传统的xxx 往往在推理时需要video token同时由于video token往往非常长，这回使得xxxx，同时我们强调虽然没有显式，但是模型依旧xxxxx

==> sections/conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}

Inthispaper,wepresentSwiftVLA, alightweight frame
workthat achievesstrongspatiotemporal reasoningwhile
maintainingdesignefficiency. Specifically,weemploya
4Dvisualgeometrytransformerwithatemporalcachethat
extracts4Dfeaturesandintegrates themintotheVLMto
enhancebothspatialandtemporalmodeling.Tobridgethe
gapbetween2Dand4Dfeatures,weintroduceFusionTo
kens,whoserepresentationsaresupervisedbythefuturetra
jectoryoftheend-effector,effectivelycapturingintegrated
multimodal information.Additionally,weemployamask
and-reconstruct strategy todistill 4Dknowledge into the
VLA,whileminimizingperformancedegradationwhen4D
inputsareomittedduringinference.Experimentsshowthat
SwiftVLAmatchestheperformanceofmodelswithupto
7×moreparameters,whileofferingupto18×fasterinfer
enceand12×smallermemoryfootprintonedgedevices.


% In this work, we presented \textit{GigaBrain-W0}, a vision-language-action model that leverages data generated by world models to overcome the scalability and diversity limitations of real-world robot data collection. By training on rich, photorealistic trajectories that span diverse scene appearances, object placements, and camera viewpoints, \textit{GigaBrain-0} achieves strong generalization across a wide spectrum of real-world robotic tasks, from dexterous manipulation to long-horizon mobile operations. Key architectural innovations, including RGBD input modeling and embodied Chain-of-Thought supervision, further enhance its spatial reasoning and sequential decision-making capabilities. Moreover, we introduced \textit{GigaBrain-0-Small}, a lightweight variant optimized for edge deployment on platforms such as the NVIDIA Jetson AGX Orin, demonstrating that VLA model can be made practical for real-time, on-device robotic control.

% Looking ahead, our work opens several promising directions for future research. First, while we currently employ world models of  video generation model as pretrained model for robot policy and explore how to pretrain the xxx to further improve. Second, we propose to use video generation as a reasoning, provide new panagdigm for World Ation models. 

% scalable \textit{data engines}, a natural next step is to integrate them as interactive \textit{policy environments} for reinforcement learning. By enabling VLA agents to roll out trajectories and receive reward signals within the world model, we could drastically reduce the need for real-world trial-and-error while supporting policy refinement through simulated experience. Second, world models may learn universal representations of physical dynamics and task structure. Such representations could allow world models to evolve beyond passive simulators into active \textit{policy generators}, capable of proposing feasible action sequences or subgoals directly. Finally, closing the loop between VLA policies and world models through self-improvement cycles—where real-world rollouts continuously refine the world model, which in turn generates better training data, could pave the way toward truly autonomous, lifelong-learning robotic systems.

% % \section{Contributors}
% % The GigaBrain-0 project is the result of collaborative efforts by a dedicated team of researchers and engineers. The contributors, listed below in alphabetical order:

% % Angen Ye,  
% % Boyuan Wang,  
% % Chaojun Ni,  
% % Guan Huang,  
% % Guosheng Zhao,  
% Haoyun Li,  
% Jie Li,  
% Jiagang Zhu,  
% Lv Feng,  
% Peng Li,  
% Qiuping Deng,  
% Runqi Ouyang,  
% Wenkang Qin,  
% Xinze Chen,  
% Xiaofeng Wang,  
% Yang Wang,  
% Yifan Li,  
% Yilong Li,  
% Yiran Ding,  
% Yuan Xu,  
% Yun Ye,  
% Yukun Zhou,  
% Zhehao Dong,  
% Zhenan Wang,  
% Zhichao Liu,
% Zheng Zhu.

==> sections/introduction.tex <==
\section{Introduction}

As a key paradigm for general-purpose robotic manipulation, Vision–Language–Action (VLA) models~\cite{pi0,pi05,go1,gr00t,gr3,walloss,galaxea,gigabrain0,swiftvla} have achieved strong performance. However, a major challenge remains: supervision sparsity. While observations and task conditioning are high-dimensional and semantically rich, action supervision is comparatively sparse and low-diversity. As a result, training objectives can become dominated by contextual signals, encouraging shortcut solutions that map many situations to a small set of action prototypes, rather than learning a continuous, compositional, and physically consistent action distribution. This reduces sample efficiency and harms generalization.



Some works~\cite{worldvla,dreamvla,swiftvla} attempt to explicitly inject future-state supervision into existing VLA frameworks by predicting intermediate signals or forecasting future observations, as illustrated in Fig.~\ref{intro}(a). Such auxiliary objectives partially alleviate the sparsity of action supervision by providing denser temporal learning signals. However, VLM-based VLA~\cite{paligemma,paligemma2,pi_0,pi05,pi06,11357220} models are typically optimized for discriminative reasoning rather than high-fidelity generation, making it non-trivial for these additional losses to translate into a continuous and physically consistent action distribution. As a result, gains in generalization and long-horizon planning are often limited. To further increase supervision density and improve scalability, recent efforts incorporate the World Model (WM) from video generation into robot policy learning~\cite{motus,lingbotva,cosmospolicy,shen2025videovla}.  Leveraging video generation is appealing because it provides temporally dense supervision in the observation space beyond sparse action labels and injects strong spatiotemporal priors learned from large-scale video data. These methods commonly optimize joint objectives of future visual dynamics and action prediction, explicitly coupling future observation forecasting with action selection, thereby leveraging the representational and generative capacity of video models to guide action learning (Fig.~\ref{intro}(b–c)). 

Despite their promise, this line of work~\cite{motus,lingbotva,cosmospolicy,shen2025videovla} has several key limitations. First, at inference time, these approaches often require generating future videos in addition to predicting actions. Since video token sequences are long, this introduces substantial computational overhead and latency, even though control only requires actions—hindering real-time deployment, particularly in high-frequency closed-loop manipulation. Second, policy performance becomes tightly coupled to video generation quality. As in Fig.\ref{intro}(b), bidirectional attention entangles action and video prediction, allowing errors to propagate across modalities; alternatively, methods in Fig.\ref{intro}(c) first generate future video and then recover actions via inverse dynamics, directly inheriting video prediction errors. Given the complexity and diversity of the real world, learning a robust open-world video generator is inherently challenging, and prediction errors can further amplify through this coupling, degrading decision quality and long-horizon stability.

\begin{figure*}[t]
    \centering
    \captionsetup{type=figure, justification=justified, singlelinecheck=false}
    \includegraphics[width=.99\linewidth]{images/intro1.pdf} 
    \vspace{-3mm}
\caption{ (a) VLM-based VLA with auxiliary future-state supervision to densify training signals, but limited by the discriminative nature of VLMs~\cite{worldvla,dreamvla,swiftvla}. (b) Joint action--video prediction with coupled attention~\cite{motus,cosmospolicy}, requiring future video generation at inference and prone to cross-modal error. (c) Two-stage design~\cite{lingbotva} that first generates future video and then gets actions via an Inverse Dynamics Model (IDM), inheriting video prediction errors and incurring additional inference cost. (d) \textit{GigaBrain-WA0}: an action-centered WAM that leverages future visual dynamics as supervision during training, but drops future-video prediction at inference for low-latency action generation.
}
    \label{intro}
    % \vspace{-2mm}
\end{figure*}

Therefore, we propose \textit{GigaBrain-WA0}, an action-centric and efficient World--Action model. Instead of making action prediction overly reliant on explicit video generation, \textit{GigaBrain-WA0} leverages future visual dynamics as a reasoning signal and a source of dense supervision. This design preserves inference efficiency while mitigating a common failure mode: control quality degrades significantly when video synthesis is imperfect. \textit{GigaBrain-WA0} is implemented as a single causal sequence model that jointly represents action tokens and future-visual tokens under a causal mask. During training, the model learns to predict future action sequences from the current observation context, while also learning to predict future visual observations conditioned on the current observation and the predicted actions. These two learning signals are optimized within the same model, allowing future visual dynamics to regularize action plausibility and provide substantially denser supervision, which improves learning efficiency and generalization. Crucially, at inference time we remove the explicit future-video prediction branch and keep only the action generation process, avoiding long video-token rollouts and enabling low-latency control, as shown in Fig.~\ref{intro}(d). To obtain stronger pretrained weights tailored to our formulation, we adopt a two-stage training pipeline. The first stage adapts the model to embodied scene representations and spatiotemporal dynamics; the second stage explicitly conditions generation on robot actions to strengthen the causal consistency between actions and visual dynamics. We also curate stage-specific datasets and leverage complementary data sources to maximize scalability and data efficiency.


% Therefore, we propose \textit{GigaBrain-WA0}, an action-centric World--Action model that leverages future visual dynamics as a reasoning signal and dense supervision, rather than making action prediction overly reliant on explicit video generation. This design preserves inference efficiency while mitigating the common failure mode where control quality degrades with imperfect video synthesis.
% \textit{GigaBrain-WA0} is implemented as a single causal sequence model that jointly represents action and future-visual tokens under a causal mask. During training, the model learns to forecast future action sequences from the current observation/task context, while also learning to predict future visual observations conditioned on the current observation and the predicted actions. These two learning signals are optimized within the same model, enabling visual dynamics to regularize action plausibility and provide substantially denser supervision. Crucially, at inference time we remove the explicit future-video prediction path and keep only the action prediction process, yielding low-latency control without long video-token rollouts.  To obtain stronger pretrained weights, we employ a three-stage training pipeline to build a robust pretraining scheme for WAM.
% We further design stage-specific curated datasets to maximize scalability and data efficiency, leveraging complementary data sources.

% The first stage adapts the video generator to embodied robotic scenes and viewpoints, improving its coverage of contact-rich interactions and domain-specific appearance. The second stage turns the model into an action-conditioned world model by injecting actions as explicit control signals, aligning predicted visual dynamics with controllable robot interactions. The final stage performs post-training on human demonstration trajectories to specialize the model for downstream manipulation.  such as task-agnostic data, synthetic data, web data, multi-robot task trajectory data, egocentric human videos, world-model generation data, and target-robot task trajectory data.


We validate \textit{GigaBrain-WA0} through experiments in real-world environments. \textit{GigaBrain-WA0} consistently outperforms strong baselines, delivering substantial efficiency gains without sacrificing control performance. On real-world robotic platforms, it runs $20\times$ faster than baseline methods, requiring only $0.2\,\mathrm{s}$ per inference, while improving task success rates by $60\%$.




The main contributions of this paper are summarized as follows:
\begin{itemize}[leftmargin=*,itemsep=2pt,topsep=2pt]
    \item We propose \textit{GigaBrain-WA0}, a unified causal sequence model that jointly represents action tokens and future visual tokens under a causal mask. During training, future visual dynamics provide dense supervision and a reasoning signal for action learning, without over-reliance on explicit video synthesis. At inference time, we drop the future-visual prediction branch and decode actions only, enabling low-latency control.
    \item We propose a pretraining paradigm that converts a generic video generation model into a strong initialization for robot policy learning, fully leveraging complementary data sources across stages.
    \item Experiments on real robotic platforms show that \textit{GigaBrain-WA0} achieves a $20\times$ inference speedup (down to $0.2\,\mathrm{s}$ per inference) while improving task success rates by $60\%$ over baseline methods.
\end{itemize}
% World Action Models (WAMs) based on large-scale pretrained video generative models have demonstrated strong capabilities in spatiotemporal world modeling and action generation. Unlike vision–language–action (VLA) models built upon pretrained vision–language models (VLMs), which often treat actions merely as output signals, WAMs first leverage video generative pretraining to learn physical regularities and motion patterns from millions of videos.  Moreover, WAMs benefit from denser supervision: during training, they are jointly constrained by action labels and visual observations, improving both action executability and spatiotemporal consistency.

% However, current WAMs face two critical bottlenecks in practical deployment. First, real-time constraints: jointly generating future pixel frames and action commands imposes substantial computational overhead, rendering inference latency prohibitive for real-time operation. Second, representation entanglement: compressing heterogeneous knowledge—high-dimensional visual semantics and low-dimensional motion commands—into a shared latent space induces information coupling. Furthermore, the tight coupling between action generation and video prediction compels excessive reliance on visual synthesis, resulting in error accumulation and decision instability that severely compromises robustness in open-world environments.
 
 
 % 一些方法为了避免 
 % 因为这些方法使用一个model来同时建模动作和未 并使用双向注意力机制


% Therefore, we propose \textit{GigaBrain-WA0}  a action-centric World-Action Model that models 2D pixel-action relationships without
% sacrificing inference efficiency and 避免action过分依赖video质量的问题. Instead of direvctlt using images to video pretrained models, we further explore how to pretrain the video generation models to better as the bases for the robot policy.  同时for traingin， 我们划分了每个阶段需要的数据 并且xxx.  We 把train the robot policy  predicting future action sequences conditioned on the current observation, and 
% generating future videos conditioned on the predicted actions and the current observation. During
% training, the model is jointly supervised by action prediction and video generation, providing rich
% learning signals and encouraging action plausibility through visual dynamics Meanwhile At inference time, we
% no longer explicitly predict future videos and retain only the action prediction process.we constrcut three stage 训练。再前面两个阶段,我们分别adpat video generation for emboied 场景和加入action作为控制条件。再第三阶段我们直接使用human demonstration数据进行后训练。




% ur approach further enhances policy robustness through two framework innovations: RGBD input modeling and embodied Chain-of-Thought (CoT) supervision. By incorporating depth information, the model gains a richer understanding of 3D geometry and spatial layout, which is crucial for precise manipulation. Meanwhile, the embodied CoT framework encourages the model to generate intermediate reasoning steps, such as manipulation trajectories and subgoal planning, mimicking the cognitive processes underlying human problem-solving. This structured reasoning enables effective handling of long-horizon tasks and fine-grained actions that require sustained attention and sequential decision-making.

% We evaluate \textit{GigaBrain-0} through extensive real-world robotic deployments, including dexterous manipulation tasks (e.g., laundry folding, paper towel preparation), long-horizon tasks (e.g., table bussing, juice preparation), mobile manipulation tasks (e.g., boxes moving, laundry baskets moving). 
% Results show that \textit{GigaBrain-0} delivers consistently strong performance across this broad range of tasks and exhibits exceptional generalization under diverse conditions, including changes in appearances (e.g., texture, color), object placements, and camera viewpoints. Furthermore, we introduce \textit{GigaBrain-0-Small}, an efficient variant optimized for deployment on hardware like the NVIDIA Jetson AGX Orin. 
% Our work highlights the potential of world model-generated data as a scalable and effective alternative to traditional data collection paradigms, marking a significant step toward versatile, general-purpose robotic systems.



==> sections/related_work.tex <==
\section{Related Works}

\subsection{World Models for Robotic Video Generation}
Recent advances in world models~\cite{recondreamer,drivedreamer4d,recondreamer++,humandreamer,humandreamerx,Recondreamer-rl,drivedreamer,mimicdreamer} have substantially improved robotic video generation and prediction~\cite{robotransfer,emma,robodreamer,cogvideo,svd,ni2025wonderfree,cogvideox,embodiedreamer}. The central goal is to learn a generative model that captures the temporal evolution of the environment, enabling the prediction of future visual sequences in either pixel space or a compact latent space. These approaches provide a scalable route for data generation, potentially mitigating data scarcity in large-scale robot learning.

Pandora~\cite{xiang2024pandora} proposes a hybrid autoregressive–diffusion world model that generates videos while enabling real-time control via free-text actions, achieving improved long-horizon consistency and controllability through large-scale pretraining and instruction tuning. FreeAction~\cite{kim2025freeaction} explicitly exploits continuous action parameters in diffusion-based robot video generation by using action-scaled classifier-free guidance to better control motion intensity and dynamics. GigaWorld-0-video~\cite{gigaworld0} is a high-fidelity world-model data engine for embodied AI that synthesizes temporally coherent, high-quality 2D video sequences with fine-grained control over appearance, scene layout, and camera viewpoints. LingBot-World~\cite{team2026advancing} is an open-source video-generation-based world simulator that supports diverse visual domains, maintains minute-level long-term consistency, and enables real-time interactive simulation.

Some methods also explore explicit video world models, which aim to construct structured and manipulable 3D scene representations~\cite{wang2025drivegen3d,wonderturbo}. Aether~\cite{team2025aether} unifies geometry-aware world modeling by jointly optimizing 4D dynamic reconstruction, action-conditioned video prediction, and goal-conditioned visual planning. Genie Envisioner~\cite{liao2025genie} builds a unified video-diffusion platform for robotic manipulation that integrates instruction-conditioned world modeling with a latent-to-action decoder and an action-conditioned neural simulator, together with a standardized benchmark for evaluation. Enerverse~\cite{huang2025enerverse} adopts a multi-view video representation with sparse long-term memory for instruction-driven future prediction, and couples generative modeling with 4D Gaussian Splatting in a data engine. GigaWorld-0-3D~\cite{team2025gigaworld} uses 3D Gaussian Splatting as the core representation to produce spatially coherent and physically grounded 3D environments, with modular components targeting reconstruction, physics, and action-related generation.


% Some metyhods also tried to  explicit video world models aim to construct structured, manipulable 3D scene representations—often leveraging multi-view imagery, depth maps, or other geometric cues. 

% GigaWorld-0-3D
% While GigaWorld-0-Video leverages video generation models to synthesize texture-rich embodied scene data,
% high-quality embodied manipulation also demands strong geometric consistency and physical accuracy. To
% address these requirements, GigaWorld-0-3D adopts 3D Gaussian Splatting (3DGS) (Kerbl et al., 2023) as
% its core scene representation, enabling the construction of spatially coherent and physically grounded 3D
% environments. Below, we detail the four key components of GigaWorld-0-3D: GigaWorld-0-3D-FG, GigaWorld-0
% 3D-BG, GigaWorld-0-3D-Phys, and GigaWorld-0-3D-Act


% In implicit video world models, the 3D scene representation is entirely encoded within the internal latent structure of the model and is not externally accessible. As a result, the evolution of the environment can only be visualized through generated video outputs. To enable action-conditioned future prediction for robotic tasks, several methods fine-tune pretrained video models on robot interaction datasets (e.g., Bridge, DROID) to generate future frames conditioned on robot actions. For instance, one approach fine-tunes the DynamicCrafter video model to support language-guided control over individual frames, enabling the synthesis of longer-horizon and more controllable videos. Another method enhances action-conditioned generation by modulating classifier-free guidance with the magnitude of input actions. Yet another extends DynamicCrafter with causal attention and diffusion forcing to achieve autoregressive action-conditioned video prediction. Additional efforts focus on object-centric dynamics modeling or generating egocentric wrist-camera views from third-person scene inputs.

% In contrast, explicit video world models aim to construct structured, manipulable 3D scene representations—often leveraging multi-view imagery, depth maps, or other geometric cues. One such method trains an autoregressive video model on simulated multi-view data conditioned on text and image inputs, producing sparse 3D reconstructions from the generated views; however, this representation may lack sufficient detail for fine-grained manipulation tasks. Another approach fine-tunes a large video model to generate depth and raymap sequences, from which a dense 3D scene geometry is recovered via back-projection. A third line of work jointly trains a video generator with an action decoder, creating a unified world model capable of action prediction, policy evaluation, and synthetic data generation—effectively bridging perception, dynamics modeling, and decision-making in a single framework.



\subsection{World Action Models for Robotic Control}
World Action Models (WAM)~\cite{cosmospolicy,motus,lingbotva,shen2025videovla}, grounded in the video generation paradigm, aim to jointly predict robot actions and future visual dynamics within a unified framework, thereby facilitating more effective robot planning and decision-making in complex environments.


% World Action Models based on video generation 范式 aim to facilitate effective robot planning and decision making coorperate with  predicting future dynamics. Existing methods are typically categorized into two classes based on their state representation.

% The first class operates in latent space  encoding task-relevant features into compact vectors and predicting their evolution through either probabilistic [36, 52, 82] or deterministic [63, 84] approaches. Representative works include the Dreamer series [12, 13, 14, 15], which perform online planning in compact latent space via Recurrent State Space Models (RSSM), significantly reducing environment interactions and computational costs. Recent advances such as the JEPA framework [27, 77] further integrate future state prediction and action generation within a unified architecture by organizing states and actions into interleaved sequences.

% The second class explicitly focuses on 2D pixel space, directly predicting future keyframes or complete video sequences [21, 33, 94, 95]. These methods model the relationship between future 2D pixel space and robot actions while directly predicting future robot observations, applying the generated actions for robot control. 
VideoVLA~\cite{shen2025videovla} directly utilizes video generation models as pretrained weights to explore the transformation of large-scale video generation models into robotic manipulation models, employing multimodal diffusion Transformers to jointly model video, language, and action modalities, achieving dual prediction of actions and future visual outcomes. Motus~\cite{motus} proposes a unified latent action world model that leverages existing general pretrained models and rich, shareable motion information, introducing a Mixture-of-Transformer (MoT) architecture to integrate three expert modules and adopting a UniDiffuser-style scheduler to enable flexible switching between different modeling modes. However, these methods typically involve massive parameter counts, making them difficult to meet the stringent requirements of real-time control.

% Moreover, this joint modeling of actions and pixels suffers from representation entanglement, where the model must compress heterogeneous knowledge ranging from high-dimensional visual semantics to low-dimensional motion commands into a shared representation space, often resulting in limited sample efficiency and suboptimal generalization performance.

To alleviate these issues, some studies have attempted autoregressive approaches. LingBot-VA~\cite{lingbotva} proposes an autoregressive video-action world modeling framework that autoregressively generates interleaved sequences of video and action representations. This method first predicts future video frames and then decodes actions through an inverse dynamics model based on predicted visual transitions. Nevertheless, such cascaded reasoning causes action prediction to heavily rely on the accuracy of video prediction. Although high-quality video imagination should theoretically correlate with reliable action prediction, constructing a precise video generation model with strong generalization capabilities is inherently extremely challenging, rendering action accuracy entirely constrained by the precision of video prediction.


